Adaptive Safety Margin Estimation for Safe Real-Time Replanning under Time-Varying Disturbance

Safe navigation in real-time is challenging because engineers need to work with uncertain vehicle dynamics, variable external disturbances, and imperfect controllers. A common safety strategy is to inflate obstacles by hand-defined margins. However, arbitrary static margins often fail in more dynamic scenarios, and using worst-case assumptions is overly conservative for most settings where disturbances over time. In this work, we propose a middle ground: safety margins that adapt on-the-fly. In an offline phase, we use Monte Carlo simulations to pre-compute a library of safety margins for multiple levels of disturbance uncertainties. Then, at runtime, our system estimates the current disturbance level to query the associated safety margins that best trades off safety and performance. We validate our approach with extensive simulated and real-world flight tests. We show that our adaptive method significantly outperforms static margins, allowing the vehicle to operate up to 1.5 times faster than worst-case static margins while maintaining safety. Video: https://youtu.be/SHzKHSUjdUU

==> __latexindent_temp.tex <==
@INPROCEEDINGS{5980229, author={L. {Meier} and P. {Tanskanen} and F. {Fraundorfer} and M. {Pollefeys}}, booktitle={2011 IEEE International Conference on Robotics and Automation}, title={PIXHAWK: A system for autonomous flight using onboard computer vision}, year={2011}, volume={}, number={}, pages={2992-2997},} 
